Joint Channel Selection and Power Control in Infrastructureless Wireless Networks: A Multi-Player Multi-Armed Bandit Framework

This paper deals with the problem of efficient resource allocation in dynamic infrastructureless wireless networks. Assuming a reactive interference-limited scenario, each transmitter is allowed to select one frequency channel (from a common pool) together with a power level at each transmission trial; hence, for all transmitters, not only the fading gain, but also the number of interfering transmissions and their transmit powers are varying over time. Due to the absence of a central controller and time-varying network characteristics, it is highly inefficient for transmitters to acquire global channel and network knowledge. Therefore a reasonable assumption is that transmitters have no knowledge of fading gains, interference, and network topology. Each transmitting node selfishly aims at maximizing its average reward (or minimizing its average cost), which is a function of the action of that specific transmitter as well as those of all other transmitters. This scenario is modeled as a multi-player multi-armed adversarial bandit game, in which multiple players receive an a priori unknown reward with an arbitrarily time-varying distribution by sequentially pulling an arm, selected from a known and finite set of arms. Since players do not know the arm with the highest average reward in advance, they attempt to minimize their so-called regret, determined by the set of players' actions, while attempting to achieve equilibrium in some sense. To this end, we design in this paper two joint power level and channel selection strategies. We prove that the gap between the average reward achieved by our approaches and that based on the best fixed strategy converges to zero asymptotically. Moreover, the empirical joint frequencies of the game converge to the set of correlated equilibria. We further characterize this set for two special cases of our designed game.

==> BEWAS-Th.tex <==
\subsection{Proof of Theorem \ref{th:NR-BEWAS}}\label{subsec:NR-BEWAS_Th}
%--------------------------------------------------------------------------------------
By Theorem \ref{th:CorrConvergence}, for every game, if no-regret strategies 
are used by all players, then the empirical joint frequencies of the game
converge to a correlated equilibrium. Therefore it suffices to show that 
the algorithm yields vanishing internal regret. To this end, we follow 
the approach of \cite{Stoltz05}, except that we apply Proposition \ref{pr:NR-BEWAS}.

Recall that by Section \ref{subsec:Conversion} and Algorithm
\ref{alg:NR-BEWAS}, the mixed strategy of each player is defined by
%
\begin{equation} 
\label{eq:deltaProbC} 
\mathbf{P}_{t}^{(k)}=\sum_{(i \to j):i\neq j}\mathbf{P}_{t}^{{(k)},(i \to j)}\delta_{(i \to j),t}^{(k)}\,.
\end{equation}
%
Hence,
%
\begin{equation} 
\label{eq:theorem}
\bar{g}^{(k)}(t,\mathbf{P}_{t})=\sum_{(i \to j):i\neq j}\bar{g}^{(k)}(t,\mathbf{P}_{t}^{(i\to j)})\delta_{(i \to j),t}\,.
\end{equation}
%
By Proposition \ref{pr:NR-BEWAS}, the external regret of Algorithm \ref{alg:NR-BEWAS} 
(NR-BEWAS) grows sublinearly in $n$. Therefore (\ref{eq:theorem}) yields 
%
\begin{equation} 
\max \sum_{t=1}^{n}\bar{g}(t,\mathbf{P}_{t}^{(i\to j)})-\sum_{t=1}^{n} \bar{g}(t,\mathbf{P}_{t}) \in o(n),
\end{equation}
%
and the definition of internal regret ensures that $\max_{i\neq j}R_{(i \to j),n} \in o(n)$, 
which concludes the proof. Details can be found in \cite{Stoltz05}, and hence are omitted.

%The proof follows the root suggested in \cite{Stoltz05}. We only give a brief review for the sake of completeness.\\
%The defining equation (\ref{eq:deltaProb}) yields
%
%\begin{equation}
%\label{eq:AuxOne}
%\sum_{i\neq j}\triangle _{(i,j),t}g_{t}(\mathbf{P}_{t}^{i \to j })=g_{t}(\mathbf{P}_{t}),
%\end{equation}
%
%where $\mathbf{P}_{t}$ is defined in (\ref{eq:probExp}). Now, using (\ref{eq:AuxOne}), and by the definition of external regret (Definition \ref{de:External}), we have
%
%\begin{equation}
%\label{eq:AuxTwo}
%\begin{aligned}
%\max_{i\neq j} g_{t}(\mathbf{P}_{t}^{i \to j })\leq& \sum_{t=1}^{n}\sum_{i\neq j}\triangle _{(i,j),t}g_{t}(\mathbf{P}_{t}^{i \to j })+R_{Ext}
%\\ 
% \leq& \sum_{t=1}^{n}\sum_{i\neq j}\triangle _{(i,j),t}g_{t}(\mathbf{P}_{t}^{i \to j })+o(n),
%\end{aligned}
%\end{equation}
%
%where the second inequality follows by Proposition \ref{pr:POne}, i.e. the fact that \textit{AEWA} yields per-round vanishing external regret. Therefore, 
%
%\begin{equation}
%\max_{i\neq j} R_{(i,j),t}\leq o(n),
%\end{equation}
%
%which completes the proof.
